Dual-Level Decoupled Transformer for Video Captioning

Video captioning aims to understand the spatio-temporal semantic concept of the video and generate descriptive sentences. The de-facto approach to this task dictates a text generator to learn from \textit{offline-extracted} motion or appearance features from \textit{pre-trained} vision models. However, these methods may suffer from the so-called \textbf{\textit{"couple"}} drawbacks on both \textit{video spatio-temporal representation} and \textit{sentence generation}. For the former, \textbf{\textit{"couple"}} means learning spatio-temporal representation in a single model(3DCNN), resulting the problems named \emph{disconnection in task/pre-train domain} and \emph{hard for end-to-end training}. As for the latter, \textbf{\textit{"couple"}} means treating the generation of visual semantic and syntax-related words equally. To this end, we present $\mathcal{D}^{2}$ - a dual-level decoupled transformer pipeline to solve the above drawbacks: \emph{(i)} for video spatio-temporal representation, we decouple the process of it into "first-spatial-then-temporal" paradigm, releasing the potential of using dedicated model(\textit{e.g.} image-text pre-training) to connect the pre-training and downstream tasks, and makes the entire model end-to-end trainable. \emph{(ii)} for sentence generation, we propose \emph{Syntax-Aware Decoder} to dynamically measure the contribution of visual semantic and syntax-related words. Extensive experiments on three widely-used benchmarks (MSVD, MSR-VTT and VATEX) have shown great potential of the proposed $\mathcal{D}^{2}$ and surpassed the previous methods by a large margin in the task of video captioning.

==> ICMR2022 (video caption) (arxiv)/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> ICMR2022 (video caption) (arxiv)/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> ICMR2022 (video caption) (arxiv)/chapters/conclusions.tex <==
\section{Conclusion}
 In this paper, we propose $\mathcal{D}^{2}$, a dual-level decoupled pure transformer pipeline for end-to-end video captioning. We address the \emph{"couple"} drawbacks on both video spatio-temporal representation learning and sentence generation. For video spatio-temporal representation, we present "first-spatial-then-temporal" paradigm. technically, we use a 2D vision transformer to generate a spatial representation for each frame and build both short and long range temporal dependency with our proposed \emph{Residual-Aware Temporal Block(RATB)}. For sentence generation, we \emph{decouple} the generation process of visual semantic and syntax-related words. Specifically, utilizing the syntactic prior provided by pre-trained language model, our proposed \emph{Syntax-Aware Decoder(SAD)} dynamically measures the contribution of visual features and syntactic prior information for the generation of each word, obtaining a more reasonable and fine-grained video captioning generation. We evaluate our methods on MSVD, MSR-VTT and VATEX, all leading to the best performance on all metrics. This sets the new state-of-the-art and our model could be the new backbone model for video captioning.
 

==> ICMR2022 (video caption) (arxiv)/chapters/exp.tex <==
\section{Experiments}
In this section, we conduct experiments to verify the effectiveness of the proposed methods. Firstly, We introduce three widely-used datasets: MSVD~\cite{chen2011collecting}, MSRVTT~\cite{xu2016msr} and recent VATEX~\cite{wang2019vatex}. Then implementation details including hyper-parameters and techniques are illustrated. After that, we make comparisons between our methods and the state-of-the-arts. More ablation studies are also discussed in the final part.

\input{tables/msrvtt_msvd}
\subsection{Datasets}
\subsubsection{MSVD}
The MSVD dataset contains 1970 video clips and roughly 80000 English sentences. It was firstly developed in 2010 and used to test and train the translational and paraphrase algorithms. Similar to the prior work~\cite{wang2019controllable}, we separate the dataset into 1,200 train, 100 validation ,and 670 test videos.

\subsubsection{MSR-VTT}
The MSR-VTT dataset contains 10,000 video clips from the YouTube website. we follow the standard splits in~\cite{xu2016msr} for fair comparison which separates the dataset into 6,513 training, 497 validation and 2,990 test videos.

\subsubsection{VATEX}
The VATEX dataset is the most recently released large-scale dataset that contains 41,269 videos. Each video is annotated with 10 English and 10 Chinese descriptions. We utilize English corpora in our experiments. According to the ofﬁcial splits~\cite{wang2019vatex}, the dataset is divided into 25,991 training, 3,000 validation, and 6,000 public testing.

\subsection{Implementation Details.}
% \subsubsection{Dataset Settings}
For the sentences longer than 30 words are truncated (50 for VATEX); the punctuations are removed (for VATEX are retained); all words are converted into lower case. 

% \subsubsection{Training Details}
Our model is trained on pixels directly via taking the frames as input. We divide video into 12 clips. If not otherwise stated, we randomly sample a single frame from each clip for training, and use the middle frame for inference. The impact of different number of clips is examined in ablation. The whole framework is optimized with ADAM~\cite{kingma2014adam} optimizer. We set the initial learning rate of the RATB and SAD to $10^{-4}$, the spatial encoder to $10^{-5}$. We pre-train our 2D visual encoder with the similar spirit as~\cite{li2021align}. For the other components, the parameters are randomly initialized with Xavier init.
Our training is started with cross entropy optimization. If the cider value drops for 5 consecutive epochs, it will turn to self-critical sequence training. The training process stops when the cider value drops for 5 consecutive epochs in self-critical sequence training.

We use input image size $256\times256$. Our model is implemented in PyTorch~\cite{paszke2019pytorch} and transformers~\cite{wolf2020transformers}.
We set the batch size to 48. The dimension of our spatial encoder is 768. We set the dimension of Residual-Aware Temporal Block and Syntax-Aware Decoder to 512. To avoid over-ﬁtting, we exploit dropout operation after the multi-head self-attention layer and the FFN of each transformer encoder layer. The dropout ratio is set to 0.1 by default. 

To guarantee the quality of generated \textit{"syntax realted features"}, we build our \textit{Syntax-Aware Encoder} based on GPT-Base provided by pytorch-transformers~\cite{wolf2020transformers}. We then fine-tune our \textit{Syntax-Aware Encoder} on caption sentences to obtain syntactic information. Fig~\ref{fig:loss} shows the validation loss and validation accuracy on VATEX datasets, demonstrating the ability of our \textit{Syntax-Aware Encoder} to encode syntactic information.
\begin{figure}[t]
\includegraphics[width =0.48\textwidth]{figure/Syntax_Encoder.pdf}
\caption{\textit{(a)}: Validation loss during Syntax-Aware Encoder fine-tuning. \textit{(b)}: Accuracy on validation set.}
\label{fig:loss}
\end{figure}
\subsection{Comparison to State-of-the-Arts}
We compare our model with the following state-of-the-art method, which all use offline feature-extractor (either 3DCNN or object detector) for spatio-temporal representation.

\begin{itemize}
    \item 
    MGSA~\cite{chen2019motion}: LSTM-based model for motion-guided caption generation.
    \item
    FCVC~\cite{fang2019fully}: Fully convolutional network for coarse-to-fine caption generation.
    \item
    POS-CG~\cite{wang2019controllable}: Part-of-speech guided caption generation. 
    \item
    POS-VCT~\cite{hou2019joint}: This method takes pos for caption generation.
    \item
    MARN~\cite{pei2019memory}: This method leverages memory network to capture cross-video contents.
    \item
    PMI-CAP~\cite{chen2020learning}: This method learns pairwise modality interactions to better exploit complementary information for each pair of modalities in video.
    \item
    SGN~\cite{ryu2021semantic}: This method uses a semantic grouping network to capture the most discriminating word phrases.
    \item
    NACF~\cite{yang2021non}: This method uses a coarse-to-fine decoding method to better capture visual words in video.
    \item
    OA-BTG~\cite{zhang2019object}: This method uses a object-aware aggregation bidirectional temporal graph (OA-BTG) to capture detailed temporal dynamics for salient objects in video. 
    \item
    GRU-EVE~\cite{aafaq2019spatio}: A LSTM based model which capture spatial-temporal dynamics by Short Fourier Transform.
    \item
    STG-KD~\cite{pan2020spatio}: This method distills the knowledge of spatial-temporal object interactions from a spatial-temporal graph.
    \item
    SAAT~\cite{zheng2020syntax}: This method learns actions by simultaneously referring to the subject and video dynamics.
    \item
    ORG-TRL~\cite{zhang2020object}: This method uses a object relation graph to build the object interactions.
    \item    OPEN-BOOK\cite{zhang2021open}:They use ``retrieval and copy" pipeline to help caption generation. 
    \item   O2NA~\cite{liuo2na}: This method uses a Object-Oriented Non-\\Autoregressive approach (O2NA). 
    
\end{itemize}
% \input{tables/msrvtt_msvd}
\input{tables/vatex}

\begin{figure*}[t]
\includegraphics[width =0.95\textwidth]{figure/showcase.pdf}
\caption{\textbf{\textit{Visualization of generations on MSR-VTT with GT and our $\mathcal{D}^{2}$}}. Compraed with baseline, our $D^{2}$ can generate more richer and descriptive captions.}
\label{showcase}
\end{figure*}

Table~\ref{msrvtt} reports the video caption performances of different models on the MSVD and MSR-VTT datasets. We can see that our $D^{2}$ consistently exhibits better performance than the others. To be specific, on MSVD, our $D^{2}$ surpasses all the other methods for all metrics by a large margin even for the strongest competitor O2NA~\cite{liuo2na}. The CIDEr-D score of our method reaches 99.2\%, which advances O2NA~\cite{liuo2na} by 2.9\%. As for MSRVTT, our $D^{2}$ achieves better performance than all the other methods for all metrics. Compared with the strongest competitor OPENBOOK~\cite{zhang2021open}, we advance it by 6.4\%(56.3 \emph{vs.} 52.9). The boost of performance on both MSVD and MSRVTT demonstrates the advantages of our $D^{2}$ which uses \emph{decoupled} pipeline on both video spatio-temporal representation learning and sentence generation. Importantly, since CIDEr-D weights the n-grams that are relevant to the video content, demonstrating that our model generates more video-relevant captions.

Besides, we also report the results of our model on the public test set of the recent published VATEX dataset as shown in Table~\ref{vatex}. Compared with these SOTA methods, our model achieves the best performance on \textit{all metrics}. Specifically, our $D^{2}$ reaches 60.9\% in terms of CIDEr-D, which advances the strongest competitor OPENBOOK~\cite{zhang2021open} by 5.9\%, proving the effectiveness of our \emph{decoupled} pipeline.

% Our full model achieve best performance on \textit{all metrics}, and the increase is particularly obvious on CIDEr-D, demonstrating the effective of proposed \textit{decoupled pipeline}.
% We found that there is a performance between previous methods and \textit{our decoupled pipeline}. Our baseline model with spatial encoder and vanilla transformer decoder has comparable performance with previous SOTA methods without the need of \textit{offline feature-extractor}, demonstrating that our new decoupled pipeline has the capability for better semantic video representation for caption generation than the widely used off-the-shelf model(3D-CNN and object detector). Our full model \textit{exceeds} all \textit{previous SOTA methods} on all datasets and all metrics. We also notice that our method have more performance gain on CIDEr-D through reinforce learning. Since CIDEr-D weights the n-grams that relevant to the video content, demonstrating that our model have more potential to obtain semantic rich video representation. 

 %This is mainly because that ~\cite{zhang2021open} use a retreval model to help decoder generate captions, it is fesiable for

\subsection{Ablation Analysis}
In this section, we conduct several ablation studies on the VATEX and MSRVTT datasets to determine some hyper-parameter and demonstrate the effectiveness of our proposed module. Since our method directly takes video frame as input and does end-to-end training; before doing the experiments about the main module, in section~\ref{sec:fps}, we first give the experiments about sample rates of input clips. Then, we give the main ablation experiments in section~\ref{sec:ablation_main} about our proposed \emph{Residual-Aware Temporal Block(RATB)} and \emph{Syntax-Aware Decoder(SAD)}. To fully exploit the effectiveness of the module in \emph{Residual-Aware Temporal Block(RATB)}, we did some experiments and give results in section~\ref{sec:temporal}. Finally, we give the ablation experiments results about image-text pre-training and end-to-end training in section~\ref{sec:backbone} and section~\ref{sec:e2e} respectively. 

\subsubsection{Ablation on number of input clips}
\label{sec:fps}
\input{tables/fps}

In order to investigate the impact of the different number of input clips, as shown in Table ~\ref{fps}, we set the number of clips to 8, 12, 16 for our model respectively. The performance cannot increase with more clips and we use 12 for our experiments.

\subsubsection{Ablation of main design of our $\mathcal{D}^{2}$}
\label{sec:ablation_main}
\input{tables/ablation_main}
 We study the benefits of RATB and SAD of our method. Specifically, the spatial encoder with image-text pre-training and vanilla transformer-based decoder are combined as our baseline model. As shown in Table~\ref{tab:my-table}, our \emph{Residual-Aware Temporal Block(RATB)} boost CIDEr score by 1.9\%(2.1\%) on VATEX(MSRVTT) dataset, demonstrating the importance of building temporal dependency for video frames. Compared Row 1 and Row 3 in Table~\ref{tab:my-table}, we observe that our \emph{Syntax-Aware Decoder(SAD)} boost CIDEr-D score from 55.2(52.1) to 57.1(53.9) on VATEX(MSRVTT) dataset, proving the effectiveness of decouple the sentence generation. Combining the above two modules, the best performance(60.9 on VATEX; 56.3 on MSRVTT) is achieved on both VATEX and MSRVTT datasets.
 
%  we first compare the performance of baseline with the state-of-the-art (\textit{openbook}). The results show that our method can obtain a competitive performance on the VATEX and MSRVTT even without external knowledge(i.e. the retrieved sentences). In row 2 and 3, we add our \textit{Residual-Aware Temporal Block}(RATB) and \textit{Syntax-Aware Decoder}(SAD) to the baseline model, we find that RATB or SAD is available as an effective sub-module and combining these two sub-modules boost the baseline performance by 2.6 (CIDEr-D) on the VATEX. Furthermore, when we integrate all module with RL, the performance improves to 64.0 (60.3) on the VATEX (MSRVTT) over the SOTA model by 11.3\% (14.0\%).


\subsubsection{Ablation of Residual-Aware Temporal Block}
\label{sec:temporal}
\input{tables/ratb}
Compared with existing methods, our Residual-Aware Temporal Block builds temporal dependency between frames in both short-range and long-range. Specifically, \textit{Residual-Level Attention(RA)} is adopted to encode short-range(atomic action) relation. Together with \textit{Temporal-Level Attention}, atomic actions in short-range segments can be contextualized with the rest of the video. Table~\ref{tab:RATB} presents the effect of two sub-modules. The results show that \textit{RA} or TA is available as an effective sub-module and combining these two sub-modules boost the CIDEr-D score by 0.9 or 1.2(1.1 or 1.4) on VATEX(MSRVTT).

\subsubsection{Ablation of image-text pre-training}
\label{sec:backbone}
\input{tables/backbone}
Due to the better accessibility of image-text datasets (as opposed to the video-text dataset, which is noisy and hard to collect), it is trivial for our spatial encoder to enrich visual semantics via pre-training on image-text pairs(\emph{e.g.}, MSCOCO). In this section, we study the effect of different types of spatial encoder and its init method. Results are summarized in Table~\ref{init}. We observed that there is a huge performance boost(row1 and row2) when replacing resnet152(cls) with ViT(cls), demonstrating that ViT has much more frame representation ability than the resnet. We hypothesize that it is mostly because the information loses via meanpooling operation~\cite{raghu2021vision}. Besides, when we conduct image-text pre-training on image-text dataset to our spatial encoder, the performance continues boosting, demonstrating that image-text pre-trained model benefits the video captioning task for its semantic spatial representation. 

\subsubsection{Ablation of End-to-End Training} \label{sec:e2e}
\input{tables/e2e}
One of the main difference between our method and previous is that we decouple the process of spatio-temporal learning: we use a 2D transformer to obtain the spatial contextual information then build temporal correlation using our designed module, giving us the benefit of end-to-end training(as opposed to 3DCNN which is hard to fine-tune). We conduct the ablation on both MSRVTT and VATEX datasets with cross-entropy loss. As it can be seen from Tab~\ref{tab:e2e}, end-to-end training boosts all metrics on MSRVTT(1.5 CIDEr score) and VATEX(2.3 CIDEr score), proving the effectiveness of our pipeline.

\subsection{Qualitative Analysis}

We show some examples in Fig.~\ref{showcase}. It can be seen, the content of captions generated by our model is richer than the baseline model, and more activity associations are involved. For instance, the example at down-left shows that the baseline model can only understand the general meaning of the video. By contrast, our model can recognize more detailed activities(\textit{e.g. } playing ping pong). The rest of the examples have similar characteristics.




==> ICMR2022 (video caption) (arxiv)/chapters/introduction.tex <==
\begin{figure}[ht!]
\includegraphics[width =0.48\textwidth]{figure/first.pdf}
\caption{\textit{Top}: The 3D-CNN or the 2D variant with complex temporal fusion block , along with an detection module to focus on the interested objects, in conventional two-stage video captioning model is generally infeasible for end-to-end finetuning due to the memory constraint on long video. \textit{Bottom}: The proposed $\mathcal{D}^{2}$ model overcomes this limit with the unified attention modules to align the language information and the decoupled spatial and temporal features which are represented by the residual coding. Benefiting from the modularized design, we can instantiate each block with dedicated pre-trained model and jointly optimize the entire system. Please refer to Fig~\ref{fig:model} for the detailed design.}
% 
\label{fig1}
\end{figure}

\section{Introduction}

\textit{Video captioning}, which aims to understand spatio-temporal relation inside the video and describe it with natural language sentences, is a fundamental research task for multi-modal video-and-language understanding. It becomes an emerging requirement with the rapid emergence of videos in our lives. To generate good captions for videos, it involves not only the understanding of spatio-temporal semantics in videos but also expressing these factors into a natural language. Existing works~\cite{zhang2020object, zhang2019object, zhang2021open, aafaq2019spatio} mainly adopt a two-stage framework for video captioning: firstly extracting visual representation of the video using offline feature extractor (3DCNN and object detector), and then decode natural sentences based on these fixed features (Fig~\ref{fig1} (top)).

Despite being reasonable, these methods still suffer from the so-called \textbf{\textit{"couple"}} drawbacks on both video spatio-temporal representation and sentence generation process. For video spatio-temporal representation, \textbf{\textit{"couple"}} means that the learning process of spatio-temporal semantic is restricted in a single model(Fig~\ref{fig1}), \emph{i.e.}, 3D CNN, which brings two main limitations: \emph{(i)} disconnection in task/pre-train domain: offline feature extractors are often trained on tasks and domains different from the target tasks. For example, 3D CNN is generally trained from pure video data without any textual input on action recognition task, while being applied to video captioning. Large-scale video-text pre-training offers a way to mitigate this issue. However, compared with its image counterpart, the collection of the video-text dataset is much more complex and its noise is also much larger~\cite{miech2020end}. This makes the video-text pre-trained models are difficult to play a big role in the video captioning tasks. Besides, convolutional kernels are speciﬁcally designed to capture short-range spatio-temporal information, they cannot model long-range dependencies that extend beyond the receptive ﬁeld. \emph{(ii)}: end-to-end training: due to the memory and computation limitation, it is also infeasible to directly plug these feature extractors into a video captioning framework for end-to-end fine-tuning, causing the disconnection between pre-trained feature and downstream tasks; For sentences generation, \textbf{\textit{"couple"}} means that existing decoding methods pay equal attention to visual semantic(\emph{"woman"} in Fig~\ref{fig1}) and syntax-related words(\emph{"are"} in Fig~\ref{fig1}) during the whole sentence generation process, making the generation process unreasonable.


To tackle the above drawbacks, we propose $\mathcal{D}^{2}$, a dual-level decoupled pure transformer pipeline for end-to-end video captioning. In terms of video spatio-temporal representation, we \emph{decouple} the learning process into "first-spatial-then-temporal" paradigm. technically, we firstly use a 2D vision transformer to generate a spatial representation for each frame, then, we propose a \emph{Residual-Aware Temporal Block(RATB)} to build the temporal relationship between each frame. This brings us two main advantages over the two limitations mentioned above: \emph{(i)}: compared to the video-text dataset, image-text dataset is easy to access, releasing the potential of applying image-text pre-training to our 2D vision transformer, which is more suitable to multimodal tasks like video captioning. \emph{(ii)} due to the lightweight nature of the 2D model (as opposed to 3D CNN), we can easily perform end-to-end training, building the connection between pre-trained feature and downstream video captioning tasks. In terms of sentence generation, we \emph{decouple} the generation process of visual semantic and syntax-related words. Concretely, using the syntactic prior provided by the pre-trained language model, our \emph{Syntax-Aware Decoder(SAD)} dynamically measures the contribution of visual features and syntactic prior information for the generation of each word, facilitating a more reasonable and fine-grained video captioning generation. %  On one hand, different from existing works, we decouple the process of spatio-temporal representation. Specifically, we use ViT-B/16 to generate features of each frames and then concate them as spatial semantic representation. Considering there is no temporal dependency between each frames, a carefully designed Residual-Aware Temporal Block(RATB) is devised to build the temporal relation at both residual and long-range level. On the other hand, during decoding stage, our Syntax-Aware Decoder(SAD) dynamically fusing semantic and syntactic features in the \textit{Syntax-Aware} attention layer, making generation of visual semantic and syntax-related words fully decoupled.

Experimentally, we conduct a series of ablation studies on different modules for \emph{decouple} spatio-temporal representation learning, as well as modules for \emph{decoupling} visual semantic and syntax-related words generation, gaining insights on the performance of our novel \emph{decouple} pipeline in video captioning task. Our \emph{$D^{2}$}, when tested on the three benchmarks(MSRVTT, MSVD and VATEX), outperforms existing methods on all metrics by a large margin. 
% The advantages of our methods are as follows: First, our method adopts a simple pipeline that does not require a complicated off-the-shelf visual backbone for spatio-temporal representation and releases the design effort for video captioning. Benefiting from the \textit{neat} and \textit{modularized} design of our pipeline, visual semantics can easily enriched by directly transfer the knowledge from dedicated pre-trained model(\textit{e.g.} image-text pre-trained model, which is more lightweight compared with its video counterpart) for end-to-end task-specific fine-tuning. Second, compared with 3D-CNN, our carefully designed Residual-Aware Temporal Block can better model long-range temporal dependency, which is quiet meaningful for video captioning. Third, we decoupled the sentence generation process for visual semantic and syntax-related words, making the whole decoding stage more reasonable.
Our main contributions are summarized as follows.% finetune 
\begin{itemize}
\vspace{-1.5mm}
\item 
We propose $\mathcal{D}^{2}$, a novel transformer pipeline, which decouple the process of \emph{video spatio-temporal representation learning} and \emph{sentence generation}. For video spatio-temporal representation learning, our pipeline decouple the previous offline spatio-temporal representation learning  into \textbf{\textit{"first spatial then temporal"}} paradigm, addressing the problems of \emph{disconnection in task/pre-train domain} and \emph{end-to-end training}.
\item 
For caption generation, our model decouples the generation of visual semantic and syntax-related words, adaptively measuring its contribution, resulting in a more reasonable and fine-grained video captioning generation process.
\item 
We show that $\mathcal{D}^{2}$ surpasses all previous methods for video captioning, achieving a new state-of-the-art on MSVD, MSR-VTT and VATEX benchmarks.
\end{itemize}


==> ICMR2022 (video caption) (arxiv)/chapters/method.tex <==
\section{Our Approach}

\begin{figure*}[t]
\includegraphics[width =1\textwidth]{figure/model.pdf}
\caption{The overall architecture of our proposed $\mathcal{D}^{2}$. $\mathcal{D}^{2}$ decouples the learning process in both video and caption side. On the video side, spatial representation is obtained using \textit{Spatial Transformer(ViT)}. With a carefully designed \textit{Residual-Aware Temporal Block}, temporal dependency is built both on \textit{residual} and \textit{long-range} level. On the caption generation side, $\mathcal{D}^{2}$ decouple the generation of visual semantic and syntax-related words by a \textit{Syntax-Aware Decoder}, in which semantic and syntactic feature is fused dynamically during the whole generation process. Benefiting from the \textit{neat} and \textit{modularized} design, we can instantiate each module with dedicated pre-trained model and jointly optimize the entire system for task-specific fine-tuning.}
\label{fig:model}
\end{figure*}

In this section, we introduce the proposed video captioning framework $\mathcal{D}^{2}$, which is illustrated in Figure~\ref{fig:model}. Compared with existing method, $\mathcal{D}^{2}$ decouple the video captioning process both in video representation and caption generation phase.  We begin with introducing the \textit{spatial encoder}. And then, the \textit{Residual-Aware Temporal Block}(RATB) and the \textit{Syntax-Aware Decoder}(SAD) are elaborated. The training details will be given at the end of this section. 

\subsection{Spatial Encoder}~\label{3.1}
Given a video $\mathcal{V}$, the video captioning task aims to generate a caption $y=\left\{y_{1}, \cdots, y_{T}\right\}$ to describe semantic concepts in $\mathcal{V}$, where $y_{t}$ denotes the $t$-th word in the caption. In the following, we introduce how a frame representation is obtained through a spatial encoder. %a transformer-based baseline model for video captioning, which eschew the offline feature-extractor in the traditional two-stage pipeline.

The video clips $v_{i}\in\mathcal{V}$ are represented as a sequence of frames (images) in our paper. Specifically, the video clip $v_{i}$ is composed of $\left|v_{i}\right|$ sampled frames such that $\left|v_{i}\right|=\left\{v_{i}^{1}, v_{i}^{2}, \ldots, v_{i}^{\left|v_{i}\right|}\right\}$. Unlike previous methods~\cite{zhang2021open, zhang2019object, wang2019controllable, zhang2020object} which extract clip features using pre-trained CNN~\cite{carreira2017quo,he2016deep} or object detector~\cite{ren2016faster}. Our $\mathcal{D}^{2}$ model is trained on pixels directly via taking the frames as input in an end-to-end manner. %Figure \ref{fig:model} demonstrates our baseline model, which mainly contains a video encoder and a vanilla transformer decoder. We will introduce each part in detail in this section.

% \subsubsection{Spatial Encoder}
In order to get the video representation, we first extract the frames from each video clip and then encode them through our spatial encoder to get a sequence of frame features. In this paper, we adopt a 2D ViT-B/16~\cite{dosovitskiy2020image} as our spatial encoder and mainly consider using a sequence of frame representation as video representation. The ViT first extracts non-overlapping image patches, then performs a linear projection to project them into 1D tokens. The transformer architecture is used to model the interaction between each patch of the input frame to get the final representation. We use the output from the [CLS] token as the frame representation. For the input frame sequence of video $v_{i}=\left\{v_{i}^{1}, v_{i}^{2}, \ldots, v_{i}^{\left|v_{i}\right|}\right\}$, the generated representation can denote as $\mathbf{Z}_{i}=\left\{\mathbf{z}_{i}^{1}, \mathbf{z}_{i}^{2}, \ldots, \mathbf{z}_{i}^{\left|v_{i}\right|}\right\}$. Benefiting from the modularized design of model, we can instantiate our spatial encoder with dedicated image-text pre-trained model. specifically, we utilize the recent one-stage image-text pre-trained model ALBEF~\cite{li2021align} to initialize our spatial encoder. The impact of different weight initialization strategies is examined in our ablation.


\subsection{Residual-Aware Temporal Block} 
\label{section:difference}
Considering that viewing video representation as a sequence of frame representations may ignore temporal dependency, we propose Residual-Aware Temporal Block(RATB) to build both long-range and Residual level temporal dependency between each frame. Since two successive frames contain content displacement, which reﬂects the actual actions, we explicitly propose a Residual Attention Mechanism to extend the input frame representation and guide the temporal transformer to encode more motion-related representations. Speciﬁcally, we adopt transformed residual of frame representation between adjacent time stamps to describe the motion change, which is formulated as:

\begin{equation}
    \mathbf{Z}_{\mathbf{d}}=\delta\left(\left\{Z_{f}^{1}-Z_{f}^{0}, Z_{f}^{2}-Z_{f}^{1}, \ldots, Z_{f}^{m-1}-Z_{f}^{m-2}\right\}+\mathbf{P}\right)
\end{equation}
where $\mathbf{P}$ is the positional embedding, $Z_{f}^{m-1}$ and $Z_{f}^{m}$ are two adjacent frame representations, $\delta$ is 1-layer transformer encoder layer, and $\mathbf{Z}_{\mathbf{d}}$ is the difference representations. We insert difference representations between every frames as below:
\begin{equation}
    \mathbf{Z}_{\mathbf{n}}=\left\{Z_{f}^{0}, Z_{d}^{1}, Z_{f}^{1}, Z_{d}^{2}, Z_{f}^{2}, \ldots, Z_{d}^{m-1}, Z_{f}^{m-1}\right\}+\mathbf{P}+\mathbf{T}
\end{equation}
where $\mathbf{Z}_{\mathbf{n}}$ is the output of our RATB, $\mathbf{P}$ is the positional embedding, $\mathbf{T}$ is the type embedding. 
With the design of residual-level attention and frame-level temporal attention, atomic actions in short term segments can be contextualized with the rest of the video, thus to be fully disambiguated. 

Compared with the 3D-CNN counterpart, which is inherently limited in capturing long-range dependencies by means of aggregation of shorter-range information, our RATB built temporal dependency at both shorter-range and long-range levels.
% \subsection{Vanilla Transforme Decoder}
% For the decoder, we use N layers of the transformer due to the advantage of its structure in text generation. Besides the self-attention as in the encoder, the decoder further adopts the cross-modal multi-head attention to compute attention weights on $\mathbf{Z}_{i}=\left\{\mathbf{z}_{i}^{1}, \mathbf{z}_{i}^{2}, \ldots, \mathbf{z}_{i}^{\left|v_{i}\right|}\right\}$ at each decoding step. Therefore, each word is generated conditioning on previously predicted words and the attended video contents.
\subsection{Syntax-Aware Decoder}
Existing decoding methods in video captioning were suffering from the semantics and syntax coupling drawback. $\mathcal{D}^{2}$  solve this problem by dynamic fusing semantic features and syntactic features during decoding. We begin with the syntactic feature extraction and then introduce the semantic and syntactic decoding method.
% Existing decoding methods in video captioning suffer from the visual and semantic couple drawback. $\mathcal{D}^{2}$ solve this problem by dynamic fusing semantic feature during decoding. We begin with the semantic feature extraction and then introduce the semantic decoding method. 
\subsubsection{Syntactic Feature Extraction}
Unlike previous works using part-of-speech(POS)~\cite{wang2019controllable} tagging tools, we choose a pre-trained language model to provide syntactic prior information. To be specific, in order to get syntactic features during the decoding stage, we build a pretrained 12-layers GPT-based language model to extract syntactic features. The language model was first pre-trained by using a large corpus of documents, and then fine-tuned by using captions sentences only. Some previous works~\cite{clark2019does} have proven that the pre-trained language model could retain syntactic information inside some of their attention heads. So in that way, we could obtain dense syntactic features containing not only POS tagging information but also the whole syntactic information by using the pretrained language model.
% In order to get semantic features during the decoding stage, we build a BERT-based language model to extract semantic features. Since the original Bert model is a stack of transformer encoder layers, which can only access previous predicated words during the test stage. Thus we add a mask self-attention layer on top of the original BERT model and design a pre-trained task to predict the future word. This simple design make our semantic encoder can provide semantic feature during test stage. 

Specifically, given the word sequence $Y$ = $\left(<\right.$bos$\left.>, {y}_{1}, {y}_{2}, \ldots, {y}_{N} \right)$, our syntax-aware encoder is asked to predict this offset sequence $\hat{Y}=\left(\hat{y}_{1}, \hat{y}_{2}, \ldots, \hat{y}_{N},<\right.$eos$\left.>\right)$ by one forward process. This entire process can be expressed as follows:
% \begin{equation}
%     hidden=BERT(Y)
% \end{equation}
\begin{equation}
    sf=\text {GPT}(Y+pos)
\end{equation}
\begin{equation}
    \hat{Y}=\log _{-} \operatorname{softmax}(FF(sf))
\end{equation}
where $pos$ is position embedding, $FF$ is feedforward network, $\hat{Y}$ is the output distribution of predicted words, $sf$ is our syntactic feature. This language model is trained with XE loss. This can be expressed as:
\begin{equation}
    sf_{t} \leftarrow SAE\left(Y_{<t}\right), sf_{t} \in \mathbb{R}^{d_{\text {model}}}
\end{equation}
where $\mathbf{SAE}$ is our Syntax-Aware Encoder.
% We train this language model with cross-entropy loss. All parameters are frozen and the output of masked attention module S is used as the representation of language features in RSTNet. This operation is formulated as:
% \begin{equation}
%     \hat{W}=\log _{-} \operatorname{softmax}(FF2(S))
% \end{equation}
\subsubsection{Visual Semantic and Syntactic Decoding}
After extracting syntactic features, we combine it with the output of our RATB as our candidates during decoding. In our opinion the visual encoder could provide more semantic information, so the decoder could choose semantic or syntactic clues flexibility by using the attention mechanism. Besides, we combine the visual encoder output features, the pretrained language model output features and the current word embedding together as the query vector of the attention module. By this way, we hope the decoder could avoid generating trivial words. This can be formulated as follows:
% After extracting semantic feature, we combine it with the output of our RATB as our candidate during decoding. This can be formulated as follows:
\begin{equation}
h_{t}=\operatorname{Decoder}\left(\left[\mathbf{Z}_{\mathbf{n}} ; sf_{t}\right], Y_{<t}\right)
\end{equation}
% During the decoding stage, visual features and semantic features are combined to generate semantic-rich captions. This can be formulated as follows:
% We build our adaptive attention module on top of the classic transformer decoder. Instead of predicting word using the hidden state h t directly, language signals introduced in Sec 3.2, visual signals output by encoder and the hidden states are combined together to measure the contribution of visual signals and language signal for each word prediction. Figure 4 depicts the the architecture of our Adaptive Attention module. The Adaptive Attention is formally deﬁne as follows:
\begin{equation}
    q_{i, t}=h_{t} W_{i}^{Q}, k_{i,t}= \left[\mathbf{Z}_{\mathbf{n}} ; sf_{t}\right] W_{i}^{K}, v_{i,t}= \left[\mathbf{Z}_{\mathbf{n}} ; sf_{t}\right]  W_{i}^{V}
\end{equation}
\begin{equation}
    \text {head}_{i, t}=\operatorname{softmax}\left(q_{i, t} k_{i, t}^{T}\right) v_{i, t}
\end{equation}
\begin{equation}
    \text {head}_{i}=\text {Concate}\left(\text {head}_{i,1}, \ldots, \text {head}_{i,M}\right)
\end{equation}
\begin{equation}
    \text {att}=\text {Concate}\left(\text {head}_{1}, \ldots, \text {head}_{h}\right) W^{O}
\end{equation}
where $\mathbf{Z}_{\mathbf{n}}$ is the output of our RATB, $sf_{t}$ is the output of syntactic encoder, $q_{i, t}$, $k_{i,t}$, $v_{i,t}$ are the query, key matrix and value matrix for the t time step word in head i respectively, ${head}_{i, t}$ is the attention result at t-th timestep, ${head}_{i}$ is the attention result in head i, att is the final attention coefficient for sequence generation.

\subsection{Training details}
The captioning model is typically trained by the cross-entropy loss (XE) given the ground-truth pair $\left(\mathcal{V}, y^{*}\right)$.

\begin{equation}
       L_{X E}(\theta)=-\sum_{t=1}^{T} \log \left(p_{\theta}\left(y_{t}^{*} \mid y_{1: t-1}^{*}, \mathcal{V}\right)\right),
\end{equation}

where $\theta$ is the parameters of our model, $y_{1: T}^{*}$ is the target ground truth sequence.

To address the exposure bias and target mismatch problem in XE, we directly optimize the non-differentiable metric with Self-Critical Sequence Training~\cite{rennie2017self}:

\begin{equation}
    L_{R L}(\theta)=-E_{y_{1: T} p_{\theta}}\left[r\left(y_{1: T}\right)\right],
\end{equation}

where the reward $r(\cdot)$ is the CIDEr-D score.

Besides, following~\cite{cornia2020meshed}, we use the mean of rewards rather than greedy decoding to baseline the reward. The gradient expression for one sample is formulated as:
\begin{equation}
    b=\frac{1}{k}\left(\sum_{i}^{k} r\left(y_{i}\right)\right),
\end{equation}
\begin{equation}
    \nabla_{\theta} L_{R L}(\theta) \approx-\frac{1}{k} \sum_{i=1}^{k}\left(\left(r\left(y_{1: T}^{i}\right)-b\right) \nabla_{\theta} \log p_{\theta}\left(y_{1: T}^{i}\right)\right),
\end{equation}
where k is the number of the sampled sequences, $y_{1: T}^{i}$ is the $i\text{-th}$, and b is the mean of the rewards obtained by the sampled sequences.


==> ICMR2022 (video caption) (arxiv)/chapters/related_works.tex <==
\section{Related Work}
\subsection{Image and Video Representation Learning With Transformer}
Inspired by the development of natural language processing, the proposed ViT~\cite{dosovitskiy2020image} firstly introduces transformer into image classification and achieves surprising performance. This motivates many researchers to conduct a more in-depth study of the transformer as the backbone network. Different from CNNs, transformers are not limited by the receptive field and can obtain more comprehensive contextual information. Meanwhile, due to the characteristics of the attention mechanism to dynamically generate attention coefficients for different instances, the expressive ability of transformers is also stronger. Considering the above advantages, researchers are increasingly applying transformers to extract feature representations, both in the field of images and videos. For the image domain, multi-scale features~\cite{Wang_2021_ICCV,Yuan_2021_ICCV, liu2021swin} are expanded by introducing pyramid structure into the transformer, allowing the transformer-based backbone to better adapt to the downstream vision tasks. Several work~\cite{liu2021swin,yuan2021volo,chu2021Twins} also focuses on the balance between attention span and computational overhead by adding local windows or filtering high-value patches.

When considering the video domain, timing information should be added. TimeSformer~\cite{bertasius2021space} studies five different variants of space-time attention and suggests a factorized space-time attention for its strong speed-accuracy trade-off. ViViT~\cite{arnab2021vivit} examines four factorized designs of spatial and temporal attention for the pre-trained ViT model. Similar to our work, they adopt divided attentions on spatial and temporal with two-path transformer models. However, they focus on patch-level attention for video action recognition. We mainly investigate frame-level spatio-temporal semantic representation for video captioning tasks. Video Swin-Transformer~\cite{liu2021video} designs a video recognition framework by transferring the thought of swin-transformer from space domain to space-time domain. Although this method has achieved certain results, the design of 3D local window still makes the overall framework complex.

The training of backbone networks often needs to be driven by a large amount of data, which usually consumes a lot of computing resources. In this paper, we design an end-to-end framework to avoid the problem of offline characterization, making the pipeline more concise.

\subsection{Video Captioning}
Over the past years, we have witnessed the great development of video captioning. Before the emergence of neural networks, template-based methods that used the concepts of Verb, Subject and Object (SVO)~\cite{barbu2012video,kojima2002natural} have become dominant. While in the era of deep learning, a broad collection of methods have been proposed ~\cite{venugopalan2014translating, ryu2021semantic} which mainly adopt an encoder-decoder framework. These works tend to extract images' features with CNNs and adopt RNNs to generate descriptions. Venugopalan~\cite{venugopalan2014translating} firstly introduces an LSTM to generate the mean pooled representations over all frames. Wang~\cite{wang2018reconstruction} tries to enhance the quality of generated captions by reproducing the frame features from decoding hidden states. And Buch~\cite{buch2017sst} connects the same output from the two hidden layers of the opposite direction at a particular time step to further refine the descriptions. However, the original implementation equipped with RNN is difficult to capture long-term dependencies since only the last hidden state takes part in the final generation. The proposed attention mechanism~\cite{gao2017video, hori2017attention, tu2017video, yao2015describing} alleviates this deficiency. For each output that the decoder generates, it has access to the entire input sequence at the temporal level. Note that different regions of each video frame also have different contributions to the prediction of the final word. For example, the description object is more important than the background. Therefore, it is also necessary to introduce spatial attention. Li~\cite{li2017mam} adopts two layers of spatio-temporal dynamic attention for video subtitles. When calculating the spatial attention weight of a specific frame, it will also consider the attention weight of the previous frame. In this way, the spatial attention map is linked across time. Wang~\cite{wang2018spotting} tries to learn a model to distinguish the foreground from the background in the video without explicit supervision, and calculates the significance score from the spatial feature map to separate the foreground and background according to the threshold. Recent work typically follows the pipeline where off-the-shelf 2D and 3D is used to extract spatio-temporal feature for video representation. Unlike previous works, we mainly focus on decouple the spatio-temporal representation learning process for better learning.

==> ICMR2022 (video caption) (arxiv)/tables/ablation_main.tex <==
\begin{table}[h!]
\centering
    \begin{tabular}{l|cc|cc|cc}
    \toprule[1pt]
    Method &
    \multicolumn{2}{c|}{Module} &
    \multicolumn{2}{c|}{MSRVTT} &
    \multicolumn{2}{c}{VATEX} \\
    \cline{2-7}
    \noalign{\smallskip}
    & RATB & SAD & B@4 & C & B@4 & C \\
    \noalign{\smallskip}\hline\noalign{\smallskip}
    Baseline &            &            &  43.3     &  52.1 & 33.9     & 55.2  \\
    Baseline & \checkmark &            & 43.9       & 54.2 & 34.2      & 57.3   \\
    Baseline &            & \checkmark & 44.1       & 53.9 & 34.4      & 57.1  \\
    Baseline & \checkmark & \checkmark & {\bf44.5}  & {\bf56.3} & {\bf35.1} & {\bf60.9}     \\
    \bottomrule[1pt]
    \end{tabular}%
\caption{\textbf{\textit{Ablation of main design of our $\mathcal{D}^{2}$}}. Spatial encoder together with vanilla decoder is selected as our baseline.}
\label{tab:my-table}
\end{table}

==> ICMR2022 (video caption) (arxiv)/tables/backbone.tex <==
\begin{table}[t]
\centering
    \begin{tabular}{lcccc}
    \toprule[1pt]
     Init Method & \multicolumn{2}{c}{MSRVTT} & \multicolumn{2}{c}{VATEX}\\
    ~              & BLEU@4  & CIDEr-D & BLEU@4  & CIDEr-D \\ 
    \hline
    Resnet152(cls)       & 27.4 & 22.6      & 17.8    & 17.2    \\
    ViT-B/16(cls)        & 40.2 & 49.2      & 29.1    & 51.4    \\
    ViT-B/16(image-text) & {\bf43.3} & {\bf52.1} & {\bf33.9}   & {\bf55.2}    \\
    \toprule[1pt]
    \end{tabular}
\caption{\textbf{\textit{Ablation study on different type of spatial encoder and different init method.}}}
\label{init}
\end{table}

==> ICMR2022 (video caption) (arxiv)/tables/e2e.tex <==
\begin{table}[h!]
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{lcccccc}
    \toprule[1pt]
    Method & \multicolumn{3}{c}{MSRVTT} & \multicolumn{3}{c}{VATEX} \\
           & BLEU@4 & METEOR & CIDEr & BLEU@4 & METEOR & CIDEr \\
    \midrule
    fix   &  43.6 & 29.2 & 54.8 & 34.3 &  24.4 & 58.6 \\
    e2e   &  44.5 & 30.0 & 56.3 & 35.1 &  25.1 & 60.9 \\
    \bottomrule[1pt]
    \end{tabular}
    }
    \caption{Ablation of the benefit of end-to-end training. }
    \label{tab:e2e}
\end{table}

==> ICMR2022 (video caption) (arxiv)/tables/fps.tex <==
\begin{table}[t]
\centering
%\scalebox{0.9} {
    \begin{tabular}{c cccc}           
    \toprule[1pt]
     Number of clips & \multicolumn{2}{c}{MSRVTT} & \multicolumn{2}{c}{VATEX}\\
    ~   & BLEU@4  & CIDEr-D & BLEU@4  & CIDEr-D \\ 
    \hline
    8  & 44.1    & 55.5    & 34.2 & 59.2    \\
    12  & {\bf44.5} & 56.3   & {\bf35.1}    & {\bf60.9}    \\
    16       & 44.3    & {\bf56.5}   & 34.3    & 60.9    \\
    
    \toprule[1pt]
    \end{tabular}
\caption{\textbf{\textit{Ablation on number of input clips}}.}
\label{fps}
\end{table}

==> ICMR2022 (video caption) (arxiv)/tables/msrvtt_msvd.tex <==
\begin{table*}[htbp]
\begin{tabular}{ l c cc cccc cccc}
\toprule[1pt]
Model  & Ref & 3DCNN & Detector& \multicolumn{4}{c}{MSVD} & \multicolumn{4}{c}{MSRVTT} \\
~ & ~ & ~ &~ & B@4 & M &R &C &B@4 & M &R &C \\
\hline
MGSA~\cite{chen2019motion} & AAAI19 & \checkmark &\small\XSolid &  53.4   & 35.0   & -       & 86.7     & 45.4   & 28.6   & -     & 50.1    \\
FCVC~\cite{fang2019fully}  & AAAI19 & \checkmark &\small\XSolid & 53.1   & 34.8   & 71.8    & 79.8     & -      & -      & -     & -       \\
POS-CG~\cite{wang2019controllable}  & ICCV19 & \checkmark &\small\XSolid & 52.5   & 34.1   & 71.3    & 88.7     & 42.0   & 28.2   & 61.6  & 48.7    \\
POS-CG+RL~\cite{wang2019controllable}       & ICCV19      & \checkmark& \small\XSolid& 53.9   & 34.9   & 72.1    & 91.0     & 41.3   & 28.7   & 62.1  & 53.4    \\
POS-VCT~\cite{hou2019joint}  & ICCV19 & \checkmark &\small\XSolid & 52.8   & 36.1   & 71.8    & 87.8     & 42.3   & 29.7   & 62.8  & 49.1    \\
MARN~\cite{pei2019memory} & CVPR19 & \checkmark &\small\XSolid & 48.6   & 35.1   & 71.9    & 92.2     & 40.4   & 28.1   & 60.7  & 47.1    \\
PMI-CAP~\cite{chen2020learning}  & ECCV20 & \checkmark &\small\XSolid & 54.7   & 36.4   & -       & 95.2     & 42.1   & 28.7   & -     & 49.4    \\
PMI-CAP+Audio~\cite{chen2020learning}    &  ECCV20    & \checkmark&\small\XSolid & -      & -      & -       & -        & 43.9   & 29.5   & -     & 50.6    \\
SGN~\cite{ryu2021semantic}       & AAAI21 & \checkmark &\small\XSolid & 52.8 & 35.5 & 72.9    & 94.3     & 40.8   & 28.3   & 60.8  & 49.5    \\
NACF~\cite{yang2021non}          & AAAI21 & \checkmark &\small\XSolid & 55.6 & 36.2 & - & 96.3 & 42.0 & 28.7 & - & 51.4    \\ \hline

OA-BTG~\cite{zhang2019object}    & CVPR19 & \checkmark &\checkmark & 56.9 & 36.2 & -     & 90.6  & 41.4 & 28.2 & -     & 46.9  \\
GRU-EVE~\cite{aafaq2019spatio}   & CVPR19 & \checkmark &\checkmark & 47.9 & 35.0 & 71.5  & 78.1  & 38.3 & 28.4 & 60.7  & 48.1  \\
STG-KD~\cite{pan2020spatio}      & CVPR20 & \checkmark &\checkmark & 52.2 & 36.9 & 73.9  & 93.0  & 40.5 & 28.3 & 60.9  & 47.1  \\
SAAT~\cite{zheng2020syntax}      & CVPR20 & \checkmark &\checkmark & 46.5 & 33.5 & 69.4  & 81.0  & 40.5 & 28.2 & 60.9  & 49.1  \\
% SAAT+RL~\cite{zheng2020syntax}   & CVPR20 & \checkmark &\checkmark & -    & -    & -     & -     & 39.9 & 27.7 & 61.2  & 51.0  \\
ORG-TRL~\cite{zhang2020object}   & CVPR20 & \checkmark &\checkmark & 54.3 & 36.4 & 73.9  & 95.2  & 43.6 & 28.8 & 62.1  & 50.9  \\
OPEN-BOOK~\cite{zhang2021open}   & CVPR21 & \checkmark &\checkmark & -    & -    & -     & -     & 42.8 & 29.3 & 61.7  & 52.9  \\
O2NA~\cite{liuo2na}              & ACL21  & \checkmark &\checkmark & 55.4 & 37.4 & 74.5  & 96.4  & 41.6 & 28.5 & 62.4  & 51.1  \\ 
\hline
$\mathcal{D}^{2}$  & -      & \small\XSolid &\small\XSolid & {\bf56.9}  &{\bf38.4}     &{\bf75.1}  &{\bf99.2}   & {\bf44.5} & {\bf30.0}    & {\bf63.3}  & {\bf56.3}     \\ 
\toprule[1pt]
\end{tabular}
\caption{\textbf{Performance comparisons on MSVD and MSRVTT benchmarks.} B@4,C,M,and R denote BLEU@4, CIDEr-D, METEOR, and ROUGE\_L, respectively. - means not available.}
\label{msrvtt}
\end{table*}

==> ICMR2022 (video caption) (arxiv)/tables/ratb.tex <==
\begin{table}[h!]
\centering
    \begin{tabular}{l|cc|cc|cc}
    \toprule[0.5pt]
    %\hline\noalign{\smallskip}
    Method &
    \multicolumn{2}{c|}{Module} &
    \multicolumn{2}{c|}{MSRVTT} &
    \multicolumn{2}{c}{VATEX} \\
    \cline{2-7}
    \noalign{\smallskip}
    & RA & TA & B@4 & C & B@4 & C \\
    \noalign{\smallskip}\hline\noalign{\smallskip}
    Baseline &            &   & 42.8 & 52.1 & 33.9 & 55.2 \\
    Baseline & \checkmark & & 43.3  & 53.2 & {\bf34.3}  & 56.1     \\
    Baseline &            & \checkmark & 43.1  & 53.5 & 34.0 & 56.4    \\
    Baseline & \checkmark & \checkmark & {\bf43.9}  & {\bf54.2} & 34.2  & {\bf57.3}     \\
    \noalign{\smallskip}\noalign{\smallskip}
    % SOTA~\cite{zhang2021open} &  &  &  & 33.9  & 57.5  & 42.8  & 52.9   \\
    \toprule[0.5pt]
    \end{tabular}
\caption{\textbf{\textit{Ablation of Residual-Aware Temporal Block}}. \textbf{\textit{RA}}, \textbf{\textit{TA}} denote \textbf{\textit{Residual-Level Attention}, \textbf{\textit{Temporal-Level Attention}}}, respectively. Spatial encoder together with vanilla decoder is selected as our baseline.}
\label{tab:RATB}
\end{table}

==> ICMR2022 (video caption) (arxiv)/tables/vatex.tex <==
\begin{table}[ht]
\centering
%\scalebox{0.65} {
    \begin{tabular}{lccccc}
    \toprule[1pt]
    Model & B@4 & M & R & C \\ \hline
    VATEX (ICCV19)~\cite{wang2019vatex} & 28.7   & 21.9   & 47.2    & 45.6    \\
    ORG-TRL (CVPR20)~\cite{zhang2020object}  & 32.1   & 22.2   & 48.9    & 49.7    \\
    NSA (CVPR20)~\cite{guo2020normalized} & 31.0   & 22.7   & 49.0    & 57.1    \\
    OPENBOOK (CVPR21)~\cite{zhang2021open} & 33.9   & 23.7   & 50.2    & 57.5    \\ \hline
    $\mathcal{D}^{2}$ &35.1   &{\bf25.1}  &{\bf51.3}  &  {\bf60.9}            \\ \toprule[1pt]
    \end{tabular}
\caption{\textbf{\textit{Performance comparisions on VATEX benchmark}}. B@4, C, M, R denote BLEU@4, CIDEr-D, METEOR, and ROUGE\_L, respectively. }
\label{vatex}
\end{table}

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC

